GEM-x: Exploration-driven Materials Discovery using Gaussian Mixtures and Ensemble Learning

Generative modeling offers a promising route to discovering crystalline materials beyond known databases, yet existing models often sample densely populated regions of composition-structure space, limiting novelty of the generated candidates. Here, we introduce GEM-x, a Gaussian mixture flow-matching framework that operates in a learned latent space and models the denoising velocity as a Gaussian mixture parametrized by a sparsely gated mixture-of-experts network, enabling multimodal, exploration-oriented sampling. We benchmark GEM-x against six leading generative models, including the All-atom Diffusion Transformer (ADiT), and assess the energetic plausibility of 1,000 generated candidates using r2SCAN density functional theory calculations. GEM-x generates stable or metastable, unique, and novel structures at a rate of 12.3%, compared with 9.6% for ADiT, representing a 28% relative improvement. This advantage is driven primarily by the generation of metastable, unique, and novel structures, for which GEM-x achieves a rate of 10.4% versus 7.1% for ADiT, a 46% relative improvement. Metastable phases are particularly attractive targets for materials discovery, as they can be experimentally realizable while offering functional properties superior to those of their thermodynamically stable counterparts. The findings suggest that exploration-driven generative modeling can expand the accessible materials landscape.

==> supp_for_main.tex <==


\clearpage

\begin{center}
    {\LARGE\bfseries Supplementary Information\par}
    
\end{center}

\vspace{0.5cm}

% Reset section, figure, table, and equation counters
\setcounter{section}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{equation}{0}

% Use SI numbering
\renewcommand{\thesection}{S\arabic{section}}
\renewcommand{\thefigure}{S\arabic{figure}}
\renewcommand{\thetable}{S\arabic{table}}
\renewcommand{\theequation}{S\arabic{equation}}



% Supporting information content
\section*{Supplementary Note 1. Training and Implementation Details}
\label{sec:supp-implementation}

% ============================================================
% 3.1 Sampling, Conditioning, and Denoising
% ============================================================

\noindent \textbf{Sampling, conditioning, and denoising.}
The sampling configuration employed for crystal generation
with GEM-x is summarized in
Supplementary Table~\ref{tab:sampling-configuration}.
The configuration includes the guidance scale,
number of generated samples, sampling batch size,
number of denoising steps, conditioning variables,
and stochastic denoising parameters.

\begin{table}[!htbp]
    \centering
    \caption{
        Sampling, conditioning, and denoising
        configuration used for GEM-x.
    }
    \label{tab:sampling-configuration}
    \begin{tabular}{ll}
        \toprule
        \textbf{Parameter} & \textbf{Value} \\
        \midrule
        Classifier-free guidance scale & 0.09 \\
        Number of samples & 1,000 \\
        Sampling batch size & 100 \\
        Number of denoising steps & 256 \\
        Dataset-index conditioning & True \\
        Space-group conditioning & True \\
        Stochastic denoising & True \\
        Noise standard deviation & 1.0 \\
        \bottomrule
    \end{tabular}
\end{table}
\FloatBarrier

% ============================================================
% 3.2 Architectural Choices
% ============================================================

\noindent \textbf{Architectural choices.} The architectural specifications of the best-performing
GEM-x model are summarized in
Supplementary Table~\ref{tab:model-architecture}.
Each expert comprises two transformer layers,
with the first operating at the model dimension
and the second at the projection dimension.
The transformer output is subsequently processed
by a multilayer perceptron (MLP) with the
specified hidden dimension. The mixture-of-experts (MoE) module comprises
eight experts, of which the top two are selected
for each input through the gating mechanism.

\begin{table}[!htbp]
    \centering
    \caption{
        Architectural specifications of the
        best-performing GEM-x model.
    }
    \label{tab:model-architecture}
    \begin{tabular}{ll}
        \toprule
        \textbf{Component} & \textbf{Value} \\
        \midrule
        Autoencoder latent dimension & 8 \\
        Model dimension & 512 \\
        Projection dimension & 1024 \\
        Number of layers & 12 \\
        Number of attention heads & 8 \\
        MLP dimension & 1,536 \\
        Dropout probability & 0.1 \\
        Number of space groups & 230 \\
        Number of Gaussian components & 8 \\
        Number of experts & 8 \\
        Top-$k$ experts & 2 \\
        \bottomrule
    \end{tabular}
\end{table}

\FloatBarrier
\noindent \textbf{Optimization and learning-rate scheduling.} The model is optimized using Adam with cosine-annealing learning-rate
decay. The corresponding hyperparameters are reported in
Table~\ref{tab:optimization-hyperparameters}.

\begin{table}[!htbp]
    \centering
    \caption{Optimization and learning-rate scheduler hyperparameters.}
    \label{tab:optimization-hyperparameters}
    \begin{tabular}{ll}
        \toprule
        \textbf{Hyperparameter} & \textbf{Value} \\
        \midrule
        Optimizer                    & Adam \\
        Initial learning rate        & $1 \times 10^{-4}$ \\
        
        Learning-rate scheduler      & Cosine annealing \\
        Scheduler frequency          & 1 \\
        Scheduler period, $T_{\max}$ & 10,000 \\
        Minimum learning rate        & $1 \times 10^{-6}$ \\
        Load-balancing coefficient   & 6 \\
        Gradient-clipping value      & 10.0 \\
        Gradient-clipping algorithm  & Norm clipping \\
        \bottomrule
    \end{tabular}
\end{table}

\FloatBarrier
\noindent \textbf{Training configuration.} Table~\ref{tab:training-configuration} provides the remaining training,
validation, logging, and hardware settings. Training beyond 4250 epochs increases validity rates, but decreases uniqueness and novelty to a point that the total percentage of VUN structures decreases, and therefore further training is no longer conducive.

\begin{table}[!htbp]
    \centering
    \caption{Training and hardware configuration.}
    \label{tab:training-configuration}
    \begin{tabular}{ll}
        \toprule
        \textbf{Parameter} & \textbf{Value} \\
        \midrule
        Minimum number of epochs          & 1 \\
        Maximum number of epochs          & 4250 \\
        Training batch size               & 128 \\
        Validation batch size             & 128 \\
        Test batch size                   & 128 \\
        Accelerator                       & GPU \\
        Number of devices                 & 8 \\
        GPU type                          & A40 \\
        Validation frequency              & Every 250 epochs \\
        Metric-logging frequency          & Every training step \\
        
        \bottomrule
    \end{tabular}
\end{table}



\FloatBarrier

\section*{Supplementary Note 2. Downstream Analysis, Structure Screening and DFT Relaxation}
\label{sec:supp-downstream}



Generated crystal structures are screened and relaxed
using the following workflow.

\begin{enumerate}

    \item \textbf{Candidate generation.}
    An initial set of 1,000 candidate crystal structures
    is generated using GEM-x.

    \item \textbf{Initial structural filtering.}
    The generated structures are evaluated for validity,
    uniqueness, and novelty. Only structures satisfying
    all three criteria are retained for subsequent screening.

    \item \textbf{Machine-learning pre-relaxation.}
    As the generated structures are not necessarily located
    at local energy minima, they are pre-relaxed using the
    pretrained SevenNet machine-learning interatomic
    potential \cite{park2024sevennet}.
    Structural relaxation is performed until the maximum
    atomic force falls below
    \SI{0.05 }{ \electronvolt\per\angstrom}.
    The pre-relaxation calculations are constructed and
    managed using the force-field workflow components
    implemented in atomate2 \cite{ganose2025atomate2}.

    \item \textbf{Initial thermodynamic-stability screening.}
    Following pre-relaxation, the energy above the
    Materials Project GGA/GGA+$U$ convex hull,
    $E_{\mathrm{hull}}^{\mathrm{GGA}}$,
    is evaluated \cite{jain2013materialsproject}.
    Structures satisfying
    \begin{equation}
        E_{\mathrm{hull}}^{\mathrm{GGA}}
        \leq 0.15~\mathrm{eV\,atom^{-1}}
        \label{eq:initial-hull-screening}
    \end{equation}
    are selected for subsequent DFT relaxation.

    \item \textbf{Magnetic-moment initialization.}
    Before performing spin-polarized DFT calculations,
    site-resolved initial magnetic moments are predicted
    using the pretrained Crystal Hamiltonian Graph
    Neural Network (CHGNet) \cite{deng2023chgnet}.
    These predictions are used to initialize the
    magnetic moments of the candidate structures.

    \item \textbf{DFT relaxation and static calculation.}
    The selected structures are evaluated using the
    \texttt{MPMetaGGADoubleRelaxStaticMaker} workflow
    implemented in atomate2 \cite{ganose2025atomate2}.
    The workflow comprises three sequential stages:
    \begin{enumerate}
        \item an initial PBEsol pre-relaxation;
        \item a higher-accuracy $r^2$SCAN structural
        relaxation; and
        \item a final $r^2$SCAN static calculation
        on the relaxed structure.
    \end{enumerate}
    The energy obtained from the final static calculation
    is used for subsequent thermodynamic-stability analysis.

    \item \textbf{Final thermodynamic-stability evaluation.}
    The final DFT energies are evaluated relative to the
    Materials Project $r^2$SCAN
    convex hull
    \cite{jain2013materialsproject,kingsbury2022mixing}.
    The resulting energy above hull,
    $E_{\mathrm{hull}}$,
    is used to classify each structure as stable,
    metastable, or unstable.

    \item \textbf{Post-relaxation uniqueness and novelty checks.}
    Uniqueness and novelty are reassessed following
    structural relaxation. This additional evaluation
    accounts for initially distinct structures that may
    converge to the same local energy minimum during
    relaxation, as well as generated structures that
    may relax to configurations already present in the
    reference dataset. Duplicate and non-novel
    structures are excluded from the final set.

\end{enumerate}

\section*{Supplementary Note 3. Additional Results}
\label{sec:supp-experimental}

This note provides additional analyses of the crystal structures
generated by GEM-x and the routing behavior of its conditional
mixture-of-experts (MoE) architecture. We examine the distribution
of crystallographic space groups among generated structures and
characterize expert routing as a function of diffusion timestep
and crystallographic space-group conditioning.



% Required packages:
% \usepackage{graphicx}
% \usepackage{subcaption}
% \usepackage{placeins}


\noindent \textbf{Timestep-dependent expert routing.} To examine how the conditional MoE architecture distributes
computation throughout the generative process, we analyze
the expert-routing weights as a function of diffusion timestep.
Supplementary Fig.~\ref{fig:moe-timestep-specialization}
presents the averaged gating-network outputs for each of
the twelve MoE layers. The heatmaps illustrate the relative contributions of
individual experts at different stages of denoising.
The timestep decreases from left to right, corresponding
to a progression from high-noise latent representations
toward low-noise representations.

\begin{figure*}[t!]
    \centering

    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/timestep_heatmaps/moe_layer_01_expert_vs_timestep.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/timestep_heatmaps/moe_layer_02_expert_vs_timestep.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/timestep_heatmaps/moe_layer_03_expert_vs_timestep.pdf}
    \end{subfigure}

    \medskip

    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/timestep_heatmaps/moe_layer_04_expert_vs_timestep.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/timestep_heatmaps/moe_layer_05_expert_vs_timestep.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/timestep_heatmaps/moe_layer_06_expert_vs_timestep.pdf}
    \end{subfigure}

    \medskip

    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/timestep_heatmaps/moe_layer_07_expert_vs_timestep.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/timestep_heatmaps/moe_layer_08_expert_vs_timestep.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/timestep_heatmaps/moe_layer_09_expert_vs_timestep.pdf}
    \end{subfigure}

    \medskip

    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/timestep_heatmaps/moe_layer_10_expert_vs_timestep.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/timestep_heatmaps/moe_layer_11_expert_vs_timestep.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/timestep_heatmaps/moe_layer_12_expert_vs_timestep.pdf}
    \end{subfigure}

    \caption{
        Timestep-dependent expert routing across the MoE layers.
        Each heatmap shows the output of the gating network, in terms of weights assigned to each expert, averaged over a batch of generated structures. Rows correspond to experts and columns correspond to diffusion
        timestep \(t\), with high-noise timesteps on the left and low-noise
        timesteps on the right. In each case, the number of called experts in sparse gating is 2.
    }
    \label{fig:moe-timestep-specialization}
\end{figure*}

\FloatBarrier

\noindent \textbf{Spacegroup-dependent expert routing.}
We further examine the dependence of expert routing on
crystallographic space-group conditioning.
Supplementary Fig.~\ref{fig:moe-spacegroup-specialization}
shows the routing weights associated with different
International space-group numbers across the twelve
MoE layers. These heatmaps provide a layer-wise characterization
of how the gating network distributes weights among
experts for different crystallographic symmetry conditions.
The visualizations complement the MoE analysis presented
in the main manuscript.

\begin{figure*}[!hbtp]
    \centering

    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/spacegroup_heatmaps/moe_layer_01_expert_vs_spacegroup.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/spacegroup_heatmaps/moe_layer_02_expert_vs_spacegroup.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/spacegroup_heatmaps/moe_layer_03_expert_vs_spacegroup.pdf}
    \end{subfigure}

    \medskip

    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/spacegroup_heatmaps/moe_layer_04_expert_vs_spacegroup.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/spacegroup_heatmaps/moe_layer_05_expert_vs_spacegroup.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/spacegroup_heatmaps/moe_layer_06_expert_vs_spacegroup.pdf}
    \end{subfigure}

    \medskip

    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/spacegroup_heatmaps/moe_layer_07_expert_vs_spacegroup.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/spacegroup_heatmaps/moe_layer_08_expert_vs_spacegroup.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/spacegroup_heatmaps/moe_layer_09_expert_vs_spacegroup.pdf}
    \end{subfigure}

    \medskip

    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/spacegroup_heatmaps/moe_layer_10_expert_vs_spacegroup.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/spacegroup_heatmaps/moe_layer_11_expert_vs_spacegroup.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
        {Figures/crystals and hulls/moe_expert_specialization/spacegroup_heatmaps/moe_layer_12_expert_vs_spacegroup.pdf}
    \end{subfigure}

    \caption{
        Space-group-dependent expert routing across the MoE layers.
        Columns correspond to the International space-group numbers and rows correspond to expert indices.  The color scale of each panel spans the
        activation range observed in that layer.
    }
    \label{fig:moe-spacegroup-specialization}
\end{figure*}




\FloatBarrier

\noindent \textbf{Space-group distribution of generated crystals.}
Supplementary Fig.~\ref{fig:spacegroup-distributions} compares
the crystallographic space-group distributions of the MP20
dataset and the structures generated by GEM-x. The generated
structures shown have undergone relaxation using SevenNet and
satisfy the metastability or stability, uniqueness, and novelty
criteria employed in the screening procedure. The distributions provide additional characterization of the
crystallographic diversity of the generated structures,
including the relative representation of different space groups.


\begin{figure}[!hbtp]
    \centering

    \begin{subfigure}[t]{1\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/spacegroup_comparison_plots/mp20_spacegroup_distribution.pdf}
        \caption{MP20 dataset}
        \label{fig:mp20-spacegroups}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{1\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/spacegroup_comparison_plots/generated_spacegroup_distribution.pdf}
        \caption{Generated samples}
        \label{fig:generated-spacegroups}
    \end{subfigure}

    \caption{
    Space-group distributions for the MP20  dataset and generated crystal structures which have been relaxed using SevenNet. After relaxation, these structures were metastable or stable,  unique and novel. Diffusion models have a tendency to over sample from the P1 spacegroup, which is the simplest spacegroup symmetry.
    }
    \label{fig:spacegroup-distributions}
\end{figure}
\clearpage

% ============================================================
% Supplementary Note 2: Mathematical Formulation of GEM-x
% ============================================================


\section*{Supplementary Note 4. Mathematical Formulation of GEM-x}
\label{sec:supp-methods}

\noindent \textbf{Unified atomic representations.} GEM-x adopts the unified atom-wise representation introduced
by the All-Atom Diffusion Transformer (ADiT)
\citep{joshi2025allatom}, which enables both periodic crystals
and non-periodic molecules to be represented in a shared
continuous latent space. This framework employs a variational
autoencoder (VAE) to map atomic structures, characterized by
categorical variables such as atomic species, and continuous
variables such as atomic positions, into continuous latent
embeddings. We use the VAE framework of ADiT to construct
the latent representation space for Gaussian-mixture flow
matching in GEM-x.

\emph{Unified representation of three-dimensional atomic systems.} An atomic system comprising $N$ atoms is described by its
atomic species $A$, Cartesian coordinates $X$, fractional
coordinates $F$, and lattice vectors $L$, defined as
\begin{equation}
\begin{aligned}
A &= \{a_i\}_{i=1}^{N} \in \mathbb{Z}^{1\times N},
&\qquad
X &= \{x_i\}_{i=1}^{N} \in \mathbb{R}^{3\times N},\\
F &= \{f_i\}_{i=1}^{N} \in [0,1)^{3\times N},
&\qquad
L &= [l_1,l_2,l_3] \in \mathbb{R}^{3\times 3}.
\end{aligned}
\label{eq:atomic-representation}
\end{equation}

For periodic crystals, the structure is fully specified
by $(A,F,L)$, with Cartesian coordinates recovered through
$X=LF$. For non-periodic molecules, the structure is
specified by $(A,X)$, while fractional coordinates and
lattice parameters are assigned a null value $\phi$.

\emph{Variational autoencoder architecture.} The VAE maps atomic structures into continuous per-atom
latent embeddings. Given the relevant structural variables,
the encoder $E$ produces
\begin{equation}
Z = E(A,X,F), \qquad
Z = \{z_i\}_{i=1}^{N} \in \mathbb{R}^{d\times N},
\label{eq:vae-encoder}
\end{equation}
where $d$ denotes the latent dimensionality, and N=20 denotes the maximum number of atoms in a crystal in MP20 dataset . The decoder
$D$ reconstructs the corresponding atomic representation,
\begin{equation}
(A',X',F',L') = D(Z).
\label{eq:vae-decoder}
\end{equation}

For periodic crystals, the reconstructed variables
$(A',F',L')$ define the periodic unit cell, whereas
for non-periodic molecules, $(A',X')$ define the
molecular structure.

\emph{Reconstruction objective.} The VAE is trained by minimizing a reconstruction loss
that quantifies the discrepancy between the reconstructed
atomic representation and the corresponding input.
A channel-wise Kullback--Leibler (KL) divergence penalty
is additionally included to regularize the latent
distribution toward a standard normal prior. For periodic crystals, the reconstruction objective
involves atomic species, fractional coordinates, and
lattice parameters. For non-periodic molecules, it
involves atomic species and Cartesian coordinates.
Further details of the VAE architecture and training
procedure are provided in Ref.~\citep{joshi2025allatom}.


\noindent \textbf{Latent flow matching.} Flow-matching generative models
\citep{lipman2023flowmatchinggenerativemodeling} transform a base distribution
into a target distribution by learning a time-dependent
vector field along an interpolation path between the
two distributions. In the latent space, this vector field
describes the flow velocity that governs the transformation
from noisy latent representations toward the latent
representations of the data.

Let $Z_{0}$ denote the clean latent representation
obtained from the VAE encoder and
$Z_{1} \sim \mathcal{N}(0,I)$ denote a sample from
the standard normal distribution. The interpolation
between these representations is defined as
\begin{equation}
Z_{t} = (1-t)Z_{0} + tZ_{1},
\qquad t \sim \mathcal{U}(0,1).
\label{eq:latent-interpolation}
\end{equation}

The corresponding ground-truth conditional vector
field is given by
\begin{equation}
u_t\left(Z_{t} \mid Z_{1}\right)
=
\frac{Z_{1}-Z_{t}}{1-t}.
\label{eq:flow-velocity}
\end{equation}

A denoising network $F$ predicts the noise endpoint
$Z'^{(1)}$ from the interpolated latent representation,
diffusion timestep, and conditioning variable:
\begin{equation}
Z'_{1} = F\left(Z_{t},t,c\right),
\label{eq:flow-denoiser}
\end{equation}
where $c$ is a binary label distinguishing periodic
and non-periodic atomic systems. The flow-matching
training objective is expressed as
\begin{equation}
\mathcal{L}_{\mathrm{fm}}
=
\frac{1}{N}
\sum_{i=1}^{N}
\frac{
\left\|Z^{(i)}_{1}-Z'^{(i)}_{1}\right\|^2
}{1-t}.
\label{eq:flow-matching-loss}
\end{equation}

\emph{Limitations of conventional flow matching.} The performance of flow-matching generative models
is influenced by several sources of error and
limitations:

\begin{enumerate}
    \item \textit{Discretization error:}
    Numerical integration of the learned ordinary
    or stochastic differential equations (ODEs/SDEs)
    introduces discretization errors.

    \item \textit{Flow-field approximation error:}
    Inaccuracies in the predicted vector field
    $u_\theta(Z_t,c)$ can arise from model underfitting.

    \item \textit{Unimodal velocity prediction:}
    A unimodal denoising velocity cannot explicitly
    represent multiple plausible trajectory endpoints
    from the same latent state.

    \item \textit{Limited sampling stochasticity:}
    When stochasticity is restricted to the initial
    sample from the base distribution, diversity
    in the generated samples may be limited.
\end{enumerate}

Reducing the integration step size can mitigate
discretization error, but increases the number of
function evaluations (NFE). Classifier-free guidance
(CFG) is commonly employed to improve conditional
predictions by combining conditional and unconditional
vector fields:
\begin{equation}
u_{\theta}^{\mathrm{CFG}}(Z_t,c)
=
w\,u_\theta(Z_t,c)
+
(1-w)\,u_\theta(Z_t),
\qquad w\in[1,\infty).
\label{eq:classifier-free-guidance}
\end{equation}

Although increasing the guidance weight $w$ can
improve alignment with the target condition,
excessive guidance may lead to out-of-distribution
latent representations.


\noindent \textbf{Forward noising process.} The forward noising process transforms a  latent
representation $Z$ into a noisy latent representation $Z_t$
according to
\begin{equation}
Z_t = \alpha_t Z + \sigma_t \varepsilon,
\qquad
\varepsilon \sim \mathcal{N}(0,I),
\label{eq:forward-noising}
\end{equation}
where $\alpha_t$ and $\sigma_t$ are predefined, time-dependent
noise-schedule coefficients.

The marginal distribution of the noisy latent variables
$p(Z_t)$ is obtained by convolving the clean latent
distribution $p(Z)$ with a Gaussian kernel. The corresponding
conditional distribution is given by
\begin{equation}
p(Z_t \mid Z_0)
=
\mathcal{N}
\left(
Z_t;\alpha_t Z_0,\sigma_t^2 I
\right).
\label{eq:forward-transition}
\end{equation}

The noise schedule satisfies the boundary conditions
\begin{equation}
Z_0 = Z,
\qquad
Z_T \approx \varepsilon.
\label{eq:noising-boundary}
\end{equation}

For the linear noising schedule, the terminal time
and schedule coefficients are defined as
\begin{equation}
T=1,
\qquad
\alpha_t=1-t,
\qquad
\sigma_t=t.
\label{eq:linear-noise-schedule}
\end{equation}


\noindent \textbf{Reverse denoising process and loss function.}
The denoising flow velocity is modeled using a Gaussian
mixture distribution,
\begin{equation}
q_\theta(u \mid Z_t)
=
\sum_{k=1}^{K}
A_{k,\theta}\,\mathcal{N}(u;\mu_{k,\theta},\Sigma_{k,\theta}),
\label{eq:gaussian-mixture}
\end{equation}
where $K$ denotes the number of mixture components,
$A_k$ is the mixture weight, and $\mu_k$ and $\Sigma_k$
denote the mean and covariance of the $k$-th component,
respectively.

The negative log-likelihood objective is defined as
\begin{equation}
\mathcal{L}
=
\mathbb{E}_{t,Z_0,Z_t}
\left[
-\log q_\theta(u\mid Z_t)
\right].
\label{eq:mixture-nll}
\end{equation}

Using an isotropic covariance parameterization,
$\Sigma_k=s^2I$, the objective can be expressed as
\begin{equation}
\begin{aligned}
\mathcal{L}
=
\mathbb{E}_{t,Z_0,Z_t}
\Bigg[
-\log
\sum_{k=1}^{K}
\exp\Bigg(
&-\frac{\|u-\mu_k(Z_t,t)\|^2}{2s^2}\\
&-D\log s
+\log A_k(Z_t,t)
\Bigg)
\Bigg],
\end{aligned}
\label{eq:mixture-nll-expanded}
\end{equation}
where $D$ denotes the dimensionality of the predicted
velocity and $s>0$ is a learned scalar shared across
mixture components. The expression omits additive
constants independent of the model parameters.

Although the isotropic covariance formulation reduces
the complexity of the mixture model, it does not
enforce a positive lower bound on the learned variance.
Consequently, the variance may approach zero during
optimization, leading to numerical instability and
large gradients.

To improve training stability, we instead adopt a
reverse-transition likelihood objective \cite{chen2025gaussian},
\begin{equation}
\mathcal{L}_{\mathrm{trans}}
=
\mathbb{E}_{t,Z_{t-\Delta t},Z_t}
\left[
-\log q_\theta
\left(
Z_{t-\Delta t}\mid Z_t
\right)
\right].
\label{eq:transition-loss}
\end{equation}

For $\Delta t<t$, the reverse-transition distribution
maintains a lower bound on its variance, which
improves numerical stability during training.

The transition time is parameterized as
\begin{equation}
t-\Delta t=\lambda t,
\qquad
\lambda\in(0,1],
\label{eq:transition-ratio}
\end{equation}
where $\lambda$ is the transition-ratio hyperparameter.

\noindent \textbf{Conditional guidance.}
The guided conditional distribution
$q_w(u \mid Z_t,c)$ is defined as
\begin{equation}
q_w(u \mid Z_t,c)
=
\frac{w(u)}{X}
q_\theta(u \mid Z_t,c),
\label{eq:guided-distribution}
\end{equation}
where $X$ denotes the normalization constant and
$w(u)$ is a Gaussian guidance mask. The guidance mask is constructed by approximating
the conditional and unconditional Gaussian-mixture
distributions with isotropic Gaussians,
$\mathcal{N}(\mu_c,s_c^2I)$ and
$\mathcal{N}(\mu_u,s_u^2I)$, respectively.
These approximations match the means and total
variances of the corresponding mixture distributions.

The guidance mask is given by
\begin{equation}
w(u)
=
\frac{
\mathcal{N}\!\left(
u;\,
\mu_c+\tilde{w}s_c\Delta\mu_n,\,
(1-\tilde{w}^2)s_c^2I
\right)
}{
\mathcal{N}\!\left(
u;\mu_c,s_c^2I
\right)
},
\label{eq:guidance-mask}
\end{equation}
where $\tilde{w}\in[0,1)$ denotes the
probabilistic guidance scale. The normalized
difference between the conditional and
unconditional means is defined as
\begin{equation}
\Delta\mu_n
=
\frac{\mu_c-\mu_u}
{\|\mu_c-\mu_u\|/\sqrt{D}},
\label{eq:normalized-mean-difference}
\end{equation}
where $D$ denotes the dimensionality of
the predicted variable $u$.


\noindent \textbf{Denoising dynamics.} Here we discuss denoising dynamics.


\emph{GM-SDE solver.} Given the predicted Gaussian-mixture distribution
$q_\theta(Z_0\mid Z_t)$, the reverse-transition
distribution can be derived analytically as
\begin{equation}
\begin{aligned}
q_\theta(Z_{t-\Delta t}\mid Z_t)
=
\sum_{k=1}^{K} A_k\,
\mathcal{N}\!\Bigl(
&Z_{t-\Delta t};\\
&c_1Z_t+c_2\mu_k,\,
(c_3+c_2^2s^2)I
\Bigr),
\end{aligned}
\label{eq:gm-sde-transition}
\end{equation}
where the coefficients $c_1$, $c_2$, and $c_3$
depend only on the noise schedule. Sampling from
this distribution yields a Gaussian-mixture
approximation to the reverse-time stochastic
differential equation (SDE).

\emph{GM-ODE solver.} The Gaussian-mixture formulation also enables
an ordinary differential equation (ODE) solver
that analytically derives the velocity field
at intermediate times without requiring
additional network evaluations.

Given $q_\theta(Z_0\mid Z_t)$, the denoising
distribution at any intermediate time $\tau<t$
is expressed as
\begin{equation}
\hat{q}(Z_0\mid Z_\tau)
=
\frac{
p(Z_\tau\mid Z_0)
}{
Z\,p(Z_t\mid Z_0)
}
q_\theta(Z_0\mid Z_t),
\label{eq:gm-ode-distribution}
\end{equation}
which remains a Gaussian mixture.
The corresponding velocity field is obtained
through reparameterization and computation
of the mixture mean, enabling low-error
integration over intermediate substeps.


\noindent \textbf{Conditional mixture of experts.} Let $G(t,c)$ denote the output of the gating network,
and let $E_i(x,t,c)$ denote the output of the $i$-th
expert network for an input representation $x$,
diffusion timestep $t$, and conditioning variable $c$.
The output $y$ of the mixture-of-experts (MoE)
module is computed as
\begin{equation}
y
=
\sum_{i=1}^{n}
G_i(t,c)\,E_i(x,t,c),
\label{eq:moe-output}
\end{equation}
where $n$ denotes the total number of experts
and $G_i(t,c)$ is the routing weight assigned
to expert $i$.

The gating weights are determined by a
top-$k$ selection operation applied to the
softmax-normalized routing logits:
\begin{equation}
G(t,c)
=
\operatorname{KeepTopK}
\left(
\operatorname{Softmax}(H(t,c)),k
\right),
\label{eq:moe-gating}
\end{equation}
where the routing logits are defined as
\begin{equation}
H_i(t,c)
=
\operatorname{MLP}_i(t,c)
+
S\,\varepsilon_i,
\qquad
\varepsilon_i\sim\mathcal{N}(0,1).
\label{eq:moe-routing-logits}
\end{equation}
The parameter $S$ controls the magnitude
of the Gaussian noise added to the routing
logits. The top-$k$ operation retains only
the selected expert weights and sets
the remaining weights to zero.
Consequently, experts for which
$G_i(t,c)=0$ need not be evaluated,
enabling sparse expert computation.




